Formal Modeling and Initial Analysis of the 4SECURail Case Study

We present the case study developed in the context of the 4SECURail project and the approach used for its formal modeling and analysis. Starting from a simple SysML/UML behavioral model of the system requirements, three formal models have been developed using three different frameworks, namely UMC, ProB, and CADP/LNT. The paper shows how the different ways to represent and analyze the system from the three different points of view allow us to take advantage of the resulting diversity.

==> eptcsdata.tex <==
\providecommand{\firstpage}{118}
\providecommand{\publicationstatus}{Clemens Dubslaff and Bas Luttik (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2022)\\
EPTCS 355, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.355.6}{10.4204/EPTCS.355.6}}
\pdfoutput=1

